Context-Aware Spectrum Coexistence of Terrestrial Beyond 5G Networks in Satellite Bands

Spectrum sharing between terrestrial 5G and incumbent networks in the satellite bands presents a promising avenue to satisfy the ever-increasing bandwidth demand of the next-generation wireless networks. However, protecting incumbent operations from harmful interference poses a fundamental challenge in accommodating terrestrial broadband cellular networks in the satellite bands. State-of-the-art spectrum-sharing policies usually consider several worst-case assumptions and ignore site-specific contextual factors in making spectrum-sharing decisions, and thus, often results in under-utilization of the shared band for the secondary licensees. To address such limitations, this paper introduces CAT3S (Context-Aware Terrestrial-Satellite Spectrum Sharing) framework that empowers the coexisting terrestrial 5G network to maximize utilization of the shared satellite band without creating harmful interference to the incumbent links by exploiting the contextual factors. CAT3S consists of the following two components: (i) context-acquisition unit to collect and process essential contextual information for spectrum sharing and (ii) context-aware base station (BS) control unit to optimize the set of operational BSs and their operation parameters (i.e., transmit power and active beams per sector). To evaluate the performance of the CAT3S, a realistic spectrum coexistence case study over the 12 GHz band is considered. Experiment results demonstrate that the proposed CAT3S achieves notably higher spectrum utilization than state-of-the-art spectrum-sharing policies in different weather contexts.

==> main_backup.tex <==
% \documentclass[10pt]{IEEEtran}
% %\documentclass[10pt, conference]{IEEEtran}
% \usepackage{graphicx}
% \usepackage{times,amsmath,amsfonts}
% \usepackage{amsmath,amssymb,amstext}
% \usepackage{multirow}
% \usepackage{hhline}
% %\usepackage{slashbox}
% \usepackage{multirow}
% \usepackage{cite}
% %\usepackage{amsmath,amssymb,amstext,mathptmx,amsfonts}
% \usepackage{epstopdf}
% \usepackage{bm}
% \usepackage{algorithm} 
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}
% %\usepackage[linesnumbered,ruled]{algorithm}
% \usepackage{color}
% %\usepackage{amsthm}
% \usepackage[lofdepth,lotdepth]{subfig}
% \usepackage{soul}
% \usepackage{float}
% %\usepackage[letterpaper, left=0.in, right=0.62in, bottom=0.598in, top=0.6in]{geometry}
% \usepackage{csquotes}
% \usepackage{xspace}


% \newtheorem{theorem}{\textbf{Theorem}}
% \newtheorem{lem}{\textbf{Lemma}}
% \newtheorem{proposition}{\textbf{Proposition}}
% \newtheorem{col}{\textbf{Corollary}}
% \newtheorem{definition}{\textbf{Definition}}

% \newcommand{\zoheb}[1]{{\color{blue}#1}}
% \newcommand{\system}{\textsf{ORCSS}\xspace}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{document}
% \title{\LARGE{Context-aware Spectrum Coexistence Design and Implementation in Satellite Bands - A Case Study of 12 GHz Band}}

% %O-RAN Enabled Context-Aware Spectrum Coexistence of Terrestrial 5G in Satellite Bands

% \markboth{Submitted Paper}%
% {Submitted Paper}
% %\author{Ta Seen Reaz Niloy, Rob Smith, Zoheb Hassan, Vikram R. Anapana, and Vijay K. Shah}


% \maketitle



% \begin{abstract}

	
    
% \end{abstract}

% \section{Introduction}
% % \begin{itemize}
% %     \item 1. In previous work we developed a digital twin to assess at a very high level the effectiveness of leveraging directionality to reduce exclusion zones
% %     \item 2. Here we enhanced that digital twin to enable codebook beamforming control (necessary to evaluate algorithms)
% %     \item 3. Proposed problem characterization and algorithm approaches
% %     \item 4. Implemented algorithms and digital twin in an O-RAN architecture
% %     \item 5. Evaluated the effectiveness of the approach for spectrum sharing and the performance of the O-RAN architecture?
    
% % \end{itemize}

% Increased capacity requirements for fifth generation (5G) and next generation networks is driving significant demand for spectrum. Pressure from industry and regulators to meet these demands means that bands with incumbent systems are being identified as candidates for spectrum sharing in the hope that cellular systems can coexist with incumbents without significant degradation to either system's performance. The effectiveness of a spectrum sharing scheme (\hl{what about the definition of effectiveness i.e. bits/s/Hz/km2}) is dependent on the flexibility of the systems in question, the potential for information sharing between these systems (context awareness), and the physical realities of the geography.

% The 12 GHz band between 12.2 - 12.7 GHz is a particularly instructional use case for the value of information sharing between systems operating in shared spectrum. Interference to non-geostationary orbit fixed satellite service (NGSO FSS), an incumbent in the band, is most impactful when the FSS antenna is aligned with the base station downlink emissions. By supplying contextual information about the FSS antenna location and pointing angle, a context-aware base station control framework can be formulated to maximize cellular system performance while meeting interference threshold targets. Additional contextual information, including RF propagation models relevant to the location of interest and current weather conditions allow base station configuration decisions to be tuned and updated over time.

% Implementing the context-aware base station control framework requires features not typically found in traditional monolithic radio access networks (RANs). Individualized control of base station beam steering parameters by an external entity and quick reaction to changes (\hl{other than changes in weather conditions, what external stimuli do we anticipate needing to react to in near-real-time?}) are particularly challenging. The emerging O-RAN network architecture promises to enable this fine-grain RAN control. The Near-Real-Time RAN Intelligent Controller (RIC) and associated E2 interface are designed for near-real-time control of base station parameters. We propose that the context-aware base station control framework is implementable as an xApp on the Near-RT RIC. Contextual information can be passed to this xApp from external sources over standard interfaces allowing the concept to be executed with minimal burden to the incumbent. The incumbent can provide a one-time indication of FSS receiver locations and pointing angles and an interface for updates to this should the need arise can be provided.


% \begin{itemize}
%     \item Motivation of spectrum sharing in the 12 GHz band (we car borrow that from the Magazine and WCL paper) (1 paragraph).

%     \item Unique challenges for spectrum sharing in the 12 GHz band and importance of context-aware spectrum sharing in the 12 GHz band (we can give an example of considering weather context in decision making, with a figure from our Magazine paper's reply) (1 paragraph).



%     \item The advantage of O-RAN to control network and hence achieving context-awareness (1 paragraph)

%     \item Novelty of our proposed approach  and contributions

%     \item Our approach leverages the directionality inherent in the antenna systems of 5G and incumbent systems. It has broad application to similar scenarios in bands where significant directionality is also useful, including:
%     \begin{itemize}
%         \item 3100 - 3550 MHz, land and mobile radar operated by US DoD
%         \item 4400 - 5000 MHz, point-to-point microwave systems
%         \item 7125 - 8500 MHz, multiple satellite and space research systems
%         \item 12.7 - 13.25 GHz, primarily Fixed Satellite Service (FSS)
%     \end{itemize}

% \end{itemize}
% As relevant government agencies research these bands they can consider the flexibility enabled by O-RAN in controlling downlink beams to minimize interference to these important 



% \textbf{Contributions of this paper.} 

% \begin{itemize}
%     \item We develop \system, an O-RAN compliant, context-aware spectrum sharing framework for enabling spectrum coexistence of 5G broadband in satellite bands, with a case study of $12$ GHz band. \system comprises two key components --(i) a \textit{context-acquisition unit} to capture important contexts (such as, weather, rf propagation model etc.), and (ii) \textit{context-aware BS control unit} as an xApp in the Near-RT RIC that determines whether a certain BS is on/off, and if on, the optimal transmitter power and operational beam at each BS sector, such that the network throughput of 5G network is maximized while maintaining the overall interference below the acceptable interference value at the NGSO FSS receiver.

%     \item We model \textit{Context-aware BS control} as a resource optimization problem aimed at dynamically optimizing three key RF parameters of the coexisting 5G network (i) set of operational 5G BSs in the shared satellite band, (ii) the active set of beams for each operation BS, and (iii) the operational transmit power of each operation BS. We showcase that the problem is NP-Hard. Following this, we propose a well-designed heuristic algorithm to obtain a sub-optimal yet computationally efficient solution to the optimization problem. This algorithm is deployed as an xApp within the Near-RT RIC of the \system system.

%     \item We design and implement \system prototype based on O-RAN Software Community Code (OSC) O-RAN Near-RT RIC, and first-of-its-kind 12 GHz interference analysis tool. Since there exists no real-world 5G deployments in $12$ GHz nor context-aware $12$ spectrum sharing/interference analysis simulation tool, we build first-of-its-kind realistic context-aware interference analysis tool~\footnote{This tool can be easily extended/modified to study other satellite bands, $6 - 40$ GHz band.} for the spectrum coexistence study of satellite bands, particularly, $12$ GHz. Following this, we integrated the 12 GHz simulation tool with O-RAN Near-RT RIC platform using E2-lite interface for the closed-loop control of base stations. 

%     \item Leveraging the \system prototype, we demonstrate the \system in the context of coexisting 5G broadband networks with NGSO FSS receivers for a semi-urban Blacksburg, VA as the case study. Experimental results show that .... 
% \end{itemize}

% \section{Related Works}

% \begin{itemize}
%     \item  Highlight DSS works in other band (e.g., CBRS) and highlight their key limitations for 12 GHz band. We can take some materials from our Magazine article and/or SWIFT proposal.

%     \item Recent works on 12 GHz band (RKF, Space-X, Direct TV, IEEE Comm Mag, and WCL)

%     \item O-RAN based spectrum sharing (Charm ) and why our work is unique compared to Charm.
%     \item Charm is all about IQ-level sensing of the spectrum and near-real-time reaction. It seems well-suited to sharing with other mobile terrestrial systems but I don't see how it adds value to this scenario where we've assumed we know what other systems are operating in the band and that we know their basic parameters. The mitigations suggested by charm are time/frequency based, not what we're looking at here

% \end{itemize}


% \section{System Overview}


% \subsection{System Model}

% \textcolor{red}{Here, we will describe the entire O-RAN based spectrum coexistence framework. We will incorporate and imporve diagram from \textbf{Vijay's} slides and explain that}

% We consider a realistic deployment scenario of $M$ number of 5G MBSs from OpenCellID database \cite{OpenCellId} and the real location of an FSS receiver which is 1770 Forecast Drive, Blacksburg, Virginia, with the latitude and longitude of  37 12’9” North and 80 26’ 4” West, respectively. The FSS receiver is positioned in the middle, creating a circle with a radius of $5000$ meters (m). From the OpenCellID database, a total of $33$ global mobile systems (GSM) MBSs are obtained within the $5000$m radius of the FSS receiver. Again, a geolocation dataset for the building of Blacksburg city is collected from OpenStreetMap by using overpass-turbo, and tota $8644$ building information is obtained from the dataset related to heights, geometric coordinates, and shapes or polygons of the buildings. 
% In terms of the height for the MBSs, we consider $10$ meters for urban-micro as per 3GPP specifications and an antenna height of $4.5$ meters for an FSS  receiver to get better signal coverage by setting it up on rooftops \cite{SpaceXanalysis}. Correspondingly the minimum and maximum heights of the buildings are considered $10$m and $40$m, respectively. The circular coverage area of each MBS with a radius $R$ is divided into $3$ equal sectors (120 degrees each) and the user equipment (UEs) are randomly placed in those sectors of the coverage region. More specifically, each MBS can support a maximum of $4$ UEs per channel considering beamforming \cite{RKFreport,SpaceXanalysis}, which means a maximum of $20$ UEs per sector can be supported by each MBS. As we consider that MBSs are 50\% loaded, thus, every MBS should transmit a signal to a total of $30$ UEs simultaneously. Here, MBSs operate using the directional antenna patterns considering 12 subarrays in 3 sectors (each housing 4 subarrays); where each subarray contains 64 predefined beam codebooks.  
% Furthermore, for the channel modeling, we consider that the MBSs can operate within the channel band of $12.2-12.7$, which is basically a total of five $100$ MHz channels for each MBS \cite{RKFreport}. In parallel, the FSS receiver operates within the band of $10.7-12.7$ GHz, consisting of eight $240$ MHz channel bandwidths that maintain a 10 MHz separation guard band. Therefore, the FSS receiver can receive data from the transmitter through these eight channels \cite{RKFreport,12GHz_WCL}. In addition, to enhance the realism of our tool, we incorporate weather-dependent environmental factors that can provide a context-aware interference analysis. Two different weather contexts: Sunny and Rainy considered here in this system. 
            

% \subsection{Proposed Framework}

% We will describe our entire proposed framework, at least consisting of two units: context-acquisition and context-aware BS control. A nice detailed figure as well as walk through of the entire framework is required.

% (i) Context-aware BS control:


% \subsection{Assumptions}
% Here we will justify our key assumptions, related to the FSS receiver's positions and pointing angles. We need to also clarify that our proposed framework can be integrated into a real system and for that we need an interference measurement report. In This paper, we consider interference measurement through a realistic simulator which provides the worst-case interference estimation. Since at present there is no setup that facilitates reporting interference from victim receiver to the O-RAN network controller, this is the best one can do. 

% \section{Proposed Method}



% \setlength{\textfloatsep}{0pt}
% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=0.95\linewidth, draft=false]{Figures/Framework.png}
% 		\caption{Proposed context-aware BS control framework.}
% 		\label{fig_2}
% 	\end{center}
% \end{figure}
% Several contextual factors, including weather conditions, RF propagation models, 5G deployment information (such as the locations and heights of BSs and buildings in the environment), and the operating parameters of incumbent receivers (such as pointing angles and positions) greatly influence the spectrum coexistence of terrestrial 5G communications in the satellite bands. By appropriately exploiting these contextual factors,  several spectrum access opportunities can be enabled for the coexisting 5G networks \cite{12GHz_ComMag}. To achieve this, in this Section, we develop a BS control framework, as shown in Fig. 1,  that effectively exploits the inherent relationship between the contextual factors and control parameters. More specifically, we first develop the realistic interference evaluation framework (Section IV. A). Subsequently, we develop an automated BS control algorithm (Section IV. B). Finally, we build the BS control unit as an O-RAN xApp by leveraging the BS control algorithm (Section IV. C).



% \subsection{Interference Evaluation Framework}

% \textcolor{blue}{We need to highlight the key features of our interference evaluation framework. Specifically, we need to highlight the inclusion of code-based beamforming and weather-dependent path loss. We also need to emphasize that this simulator provides us with a flexible tool to analyze the impact of various ``what-if'' scenarios/policies and select the best policy.}

% \subsubsection{Transmitter Antenna Pattern of 5G MBS}:
% 5G MBSs use a ($M \times N$) Planar Array antenna for the codebook-based beamforming towards the UEs in each sector within its coverage area; where $M$ and $N$ are the numbers of rows and columns of the antenna element's array. The spacing between antenna elements along the $x$ and $y$ axes is denoted as $d_x$ and $d_y$, respectively, which is calculated as $\lambda/2$ (where $\lambda$ is the wavelength). Progressive phase shifts are introduced as $\beta_x$ and $\beta_y$. In this context, $12$ subarrays within $3$ sectors are considered where each sector is equipped with $4$ subarrays and each subarray consists of a total of 64 predefined beam codebooks. For shaping the beams by taking into account the antenna array configuration, antenna elements spacing, and antenna array size, we leverage the planner antenna array factor in \cite{Balanis} for specific azimuth and elevation angles $\theta \in [0, \pi]$ and $\phi \in [-\pi, \pi]$.

% \begin{equation} \label{eq:euation_AF}
% AF_{m}(\theta, \phi) = 
% \left.\begin{cases} \frac{1}{M}\frac{Sin(\frac{M}{2}\psi_{x})}{Sin(\frac{\psi_{x}}{2})}\end{cases}\right\}
% \left.\begin{cases} \frac{1}{N}\frac{Sin(\frac{N}{2}\psi_{y})}{Sin(\frac{\psi_{y}}{2})}\end{cases}\right\}
% \end{equation}

% Furthermore, the phase differences  $\psi_{x}$ and $\psi_{y}$ for the $k$-th wave number are expressed as:
% \begin{equation}
% \psi_{x} = kd_{x} sin\theta cos\phi + \beta_{x}
% \end{equation}
% and 
% \begin{equation}
% \psi_{y} = kd_{y} sin\theta cos\phi+ \beta_{y} 
% \end{equation}
% We assume that one beam in one sector of a particular MBS can be operational based on the best power and best codebook weight. Therefore, The overall antenna gain of that beam in dB scale for the $m$-th subarray and $\phi$-the azimuth angle and $\theta$-th elevation angle which is directed towards the $i$-th UE is calculated as \eqref{eq:euation_gain}
% \begin{equation} \label{eq:euation_gain}
% G_{5G}^{(i)}(\theta, \phi) = 10 \log[AF({m},{\phi},{\theta})]
% \end{equation}


% \subsubsection{Receiver Antenna Pattern of FSS}: The Class B wide band earth stations (WBES) antenna pattern is considered on the receiver side, which ETSI standardizes. Similar to the recent interference analysis on 12GHz satellite band \cite{12GHz_WCL}, this research involves the utilization of Equation \eqref{eq:IN_equation_fss} to compute antenna gain for specific $\phi$ angles relative to the boresight direction.
%    \begin{equation} \label{eq:IN_equation_fss}
%    G_{FSS}(\phi) =
%    \begin{cases}
%    40- 25 \log \phi ~ \text{dBi} & 6^{\circ} \leq \phi < 48^{\circ}\\
%    -2 ~  \text{dBi} & 48^{\circ} \leq  \phi \leq 180 ^{\circ}.
%    \end{cases}
%    \end{equation}

% \subsubsection{Path Loss Model}:
% In this work, we employ a site-specific and weather-dependent path loss model to accurately compute the Line-of-sight (LOS) and Non-Line-of-sight (NLOS) propagation paths. Unlike the probabilistic method \cite[Table 7.4.2]{pathloss}, our model takes into account various factors, including distance ($d_k$) between MBSs and Users, building heights, building polygons, and weather-specific phenomena (sunny and rainy). We start by integrating building information, including their heights, geographical coordinates, and shapes, obtained from the OpenStreetMap database within an inclusion zone of $5000$ meters. Based on the geolocation of MBSs and the FSS receiver, we determine, whether any building polygons are intersected by the MBS and FSS receiver's interference axis; if an intersection is present, we classify the link between an MBS and the FSS receiver as Line-of-Sight (LOS); otherwise, it is Non-Line-of-Sight (NLOS) \cite{12GHz_WCL}. Moreover, for modeling the sunny weather propagation loss (dB unit), the following equation \eqref{PL} is utilized by considering the distance $d_k$ between the $k$-th interfering MBS to FSS receiver\cite{Hattab2018InterferenceAO}.
%  \begin{equation}
%      \label{PL}
%      \begin{split}
%     &     \text{PL}(d_k)_{(Sunny)}= \mathbf{1}_{(\beta=0)}\left(\text{PL}_{\mbox{\tiny{NLOS}}}(d_k)+X(\sigma_{\mbox{\tiny{NLOS}}})\right)\\
%   &  + \mathbf{1}_{(\beta=1)}\left(\text{PL}_{\mbox{\tiny{LOS}}}(d_k)+X(\sigma_{\mbox{\tiny{LOS}}})\right)\
%      \end{split}
%  \end{equation}

%  Here, $\beta\in \{0,1\}$ signifies that $\beta=0$ corresponds to the NLOS propagation $\text{PL}_{\mbox{\tiny{NLOS}}}(d_k)$, while $\beta=1$ denotes the LOS propagation scenario $\text{PL}_{\mbox{\tiny{LOS}}}(d_k)$ with an indicator function $\mathbf{1}_{(\cdot)}$. The shadow fading loss (in dB) is represented as $X(\sigma_{\mbox{\tiny{b}}})$, where $\sigma_b$ is the standard deviation for $b \in \{\mbox{LOS, NLOS}\}$. We leverage the 3GPP path loss models, \cite[Table 7.4.1]{pathloss} for the values of $\text{PL}_{\mbox{\tiny{NLOS}}}(d_k)$ and $\text{PL}_{\mbox{\tiny{LOS}}}(d_k)$. 
 
%  Additionally, for rainy weather-specific path loss modeling, we incorporate an additional term Attenuation Factor due to Rain in \eqref{PLW}:
%  \begin{equation}
%     \label{PLW}
%     \text{PL}(d_m)_{(Rainy)} =\text{PL}(d_m)_{(Sunny)}+ \text{A}_{Rain}
%     \end{equation}

% The mathematical model Rain Wave Attenuation due to Rain (RWAR) is utilized for predicting rain-induced attenuation ($A$) in dB/Km, which is applicable for both vertical and horizontal polarizations with a frequency range of 10 GHz to 100 GHz \cite{PL_Rain}.
% \begin{equation}
%     \label{AF}
%     \begin{split}
%     & A(\frac{dB}{{Km}})= af^3+ bf^2+ cf+d
%     \end{split}
%     \end{equation}
% Here, constants $a$, $b$, $c$, and $d$ are determined through a curve fitting algorithm for vertical polarization using \eqref{a},\eqref{b},\eqref{c},\eqref{d}, as detailed in \cite{PL_Rain}; while the rain rate ($x$) in mm/h is obtained from the OpenWeatherMap API which provides weather information of a specific day for particular geolocation or city.

% \begin{equation}
%     \label{a}
%     \begin{split}
%     a = -5.520\times10^{-12} x^3 + 3.26\times10^{-9} x^2\\
%     - 1.21x\times 10^{-7} - 6\times 10^{-6} 
%     \end{split}
%     \end{equation}
% \begin{equation}
%     \label{b}
%     \begin{split}
%     b = 8\times10^{-10} x^3 - 4.522\times10^{-7} x^2 
%     - 3.03x\times 10^{-5} \\+ 0.001
%     \end{split}
%     \end{equation}

%     \begin{equation}
%     \label{c}
%     \begin{split}
%     c = -5.71\times10^{-9} x^3 + 6\times10^{-7} x^2
%     +8.707x\times 10^{-3} \\- 0.018
%     \end{split}
%     \end{equation}
% \begin{equation}
%     \label{d}
%     \begin{split}
%     d = -1.073\times10^{-7} x^3 + 1.068\times10^{-4} x^2\\
%     -0.0598x\times 10^{-3} +0.0442
%     \end{split}
%     \end{equation}

% \subsubsection{Channel Model}: As discussed in the recent work of $12$GHz band \cite{12GHz_WCL} both FSS receiver and terrestrial 5G operation coexist within $12.2-12.7$ GHz band through two distinct channels of the FSS receiver specified as FSS-CH-1($12.2-12.45$GHz) and FSS-CH-2($12.45-12.7$ GHz). Simultaneously, the downlink operation of MBS takes place within this band by dividing into five distinct channels, each having a bandwidth of 100 MHz: (i) CH-1($12.2-12.3$ GHZ), (ii) CH-2($12.3-12.4$ GHZ), (iii) CH-3($12.4-12.5$ GHZ), (iv) CH-2($12.5-12.6$ GHZ) and (v) CH-2($12.6-12.7$ GHZ). We denote the total set of UEs within the coverage area of the $m$-th MBS as $U$. Additionally, $U$ can be divided into two subsets: $U_1$, which includes UEs scheduled in CH-1, CH-2, and CH-3, and $U_2$, which incorporates UEs scheduled in CH-3, CH-4, and CH-5. As discussed in the previous section, each sector of a particular MBS can operate one beam depending on the best power and best codebook weight towards the UE. Hence, it is the scheduling of UEs on these channels that dictates a group of interfering beams. Consequently, the aggregation of interference beams $U_k$ originating from MBSs is influenced by the scheduling and operation of UEs across these designated channels \eqref{Channel}.
% \begin{equation}
%     \vspace{-0.2cm}
%     \label{Channel}
%     \begin{split}
%     \mathcal{U}_k=\begin{cases}
%     \mathcal{U}, & \mbox{Both FSS-CH-1 and FSS-CH-2 are active}\\
%     \mathcal{U}_1, & \mbox{Only FSS-CH-1 is active}\\
%     \mathcal{U}_2, & \mbox{Only FSS-CH-2 is active}
%     \end{cases}
%     \end{split}
% \end{equation}

% \subsubsection{Evaluation of Aggregated Interference}: The received interference power (in dB unit) at the incumbent satellite receiver created by the $n$-th directional beam transmitted from $m$-th sub-array of the $k$-th BS is expressed as
% \begin{equation}
%     \label{SINR_u_k}
%     \begin{split}
%     I_{k,m,n}= & 10\log_{10}(P_k)+ G_{5G}^{(k)}\left(\theta_{n,int}, \phi_{n,int}\right)+ G_{SAT}(\phi_{k, SAT})\\
%     & -\text{PL}(d_{k,SAT})-10\log_{10}(M)\\
% \end{split}
% \end{equation}

% where $G_{5G}^{(n)}\left(\cdot\right)$ is the antenna gain function of the BS; $G_{5G}^{(k)}(\cdot)$ is the antenna gain function of the $k$-th BS; $G_{SAT}(\cdot)$ is the antenna gain function of the incumbent satellite receiver; $\theta_{n,int}$ and $\phi_{n,int}$ are the azimuth and elevation angles between the interference axis (from the $k$-th BS to the satellite receiver) and the $n$-th transmitted beam, respectively;  $\phi_{k, SAT}$ is the angle between incumbent receiver's boresight direction and interference axis from the $k$-th BS; $\text{PL}(\cdot)$ is the path loss in dB unit with $d_{k, SAT}$ as the distance between the $k$-th BS and satellite receiver.  Thereby, the aggregated interference received from  the $k$-th BS to the incumbent satellite receiver is obtained as
% \begin{equation}
%     \label{interfernece}
%     I_k=\sum_{m=1}^M\sum_{n=1}^{N}  z_{k,n}^{(m)} 10^{\frac{I_{k,m,n}}{10}}.
% \end{equation}



% \subsection{BS Control Algorithm}
% %Here, we need to describe our control algorithms. We can present problem formulation, prove NP-hardness, and then describe the algorithm. We also need to present computational complexity.
% In this section, we present and solve a resource optimization problem aimed at dynamically controlling three key RF parameters of the coexisting 5G cellular network, namely, (i) the set of operational 5G BSs in the shared satellite band, (ii) the active set of beams for each operational BS, and (iii) the operating transmit power of each operational BS. Our objective is to maximize the utilization of the satellite band for the coexisting 5G cellular network while ensuring interference protection for incumbent satellite receivers. 
% In what follows, we first present the optimization problem and analyze its properties. Subsequently, we develop a heuristic algorithm to obtain a sub-optimal yet computationally efficient solution to this optimization problem.

% \subsubsection{Optimization Problem Formulation}
% We first introduce the optimization and system variables. We assume that there are a total of $K$ 5G BSs in the considered region, and $\mathcal{K}=\{1,2, \cdots, K\}$ be the set of all BSs. Let $\nu_k \in \{0,1\}$ be the BS activation indicator where $\nu_k=1$ implies that the $k$-th BS is operational in the shared satellite band, and otherwise, $\nu_k=0$.  Each BS has a total of $M$ number of sub-arrays, each being fed with an RF chain and there are a total of $N$ unique codebook vectors for each sub-array, each representing a unique 3D beam direction\footnote{This work considers a codebook-based multi-user MIMO beamforming technique, where each BS can form at most $M$ beams in different directions. In practice, this is accomplished by loading suitable codebook vectors at different sub-arrays of a BS.}. Let  $\mathcal{N}_{k}^{(m)}= \{1,2 \cdots, N\}$ be the set of codebook vectors  transmitted from the $m$-th sub-array of the $k$-th BS. We introduce a binary variable $z_{k,m}^{(n)} \in \{0,1\}$ where $z_{k,m}^{(n)}=1$ means that the  $n$-th codebook vector is loaded to the $m$-th sub-array of the $k$-th BS and otherwise, $z_{k,m}^{(n)}=0$.

% %$Moreover, we assume that the $k$-th BS transmits a total of $N_k$ beams obtained from the codedbook based beam selection algorithm provided in the previous section. We denote $\mathcal{K}=\{1,2, \cdots, K\}$ and $\mathcal{N}_k= \{1,2 \cdots, N_k\}$ by the set of total BSs and the set of beams transmitted from the $k$-th BS, respectively.  We introduce another binary variable $z_{k,n} \in \{0,1\}$ where $z_{k,n}=1$ means that the $n$-th transmitted beam from the $k$-th BS is active in the shared satellite band and otherwise, $z_{k,n}=0$\footnote{We assume that the considered BSs have multi-band transmission capability, i.e., they can simultaneously transmit in both the considered satellite and sub-6 GHz bands. Therefore, if a beam is not allowed to be active in the considered satellite band, BS can transmit this beam using the sub-6 GHz band. The dual band BSs with the capability of transmitting  in both mmWave and sub-6 GHz bands are available for current 5G deployments, and we expect that it would be the same when 5G will be deployed in the satellite mid-bands.}.  

% We denote  the achievable capacity of the $k$-th BS in downlink by $C_k$ and the beam created by loading the $n$-th codebook vector at the $m$-th sub-array covers a total $F_{k,n}^{(m)}$ number of UEs. From the codebook based beam forming algorithm presented in Section III. A, we can readily determine $F_{k,n}^{(m)}, \forall k,n,m$. Without loss of generality, we assume that the total transmitted power from each BS is equally divided among the sub-arrays.  Let us consider that the $u$-th UE is supported by the $n$-th beam transmitted from the $k$-th BS's $m$-th sub-array. The received SNR (in the unit of dB) at the $u$-th UE  is expressed as
% \begin{equation}
%     \label{SINR_u_k}
%     \begin{split}
%     \text{SNR}_{k,m,n}^{(u)}= & 10\log_{10}(P_k)+ H^{(m,n)}\left(\Theta_{n}, \Theta_u\right)-\text{PL}(d_{k,u})\\
%     &-10\log_{10}(NP)-10\log_{10}(M)
% \end{split}
% \end{equation}
% where $P_k$ is the transmitted power from the $k$-th BS in Watt; $H^{(m,n)} (\Theta_{n}, \Theta_u)$ is the overall antenna gain (in dBi unit) from the $n$-th beam towards the $u$-th UE with $\Theta_n$ and  $\Theta_u$ as the angle-of-departure and angle-of-arrival, respectively; $\text{PL}(d_{k,u})$ is the path loss (in dB unit) with $d_{k,u}$ as the distance between the $k$-th BS and $u$-th UE; and $\text{NP}$ is the noise power in Watt. The achievable downlink capacity (in bps/Hz unit) at the $u$-th UE  is obtained as $C_{k,m,n}^{(u)}=\log_2\left(1+10^{SNR_{k,m,n}^{(u)}/10}\right)$. Therefore, the total achievable downlink capacity of the $k$-th BS is obtained as\footnote{We consider that BSs select their electric downtilt angles to minimize the inter-cell interference, and thus, the inter-cell interference is ignored. At the same time, due to spatial and angular distance, the intra-cell interference between two concurrently active beams (using the same frequency channels) at different sectors is also considered to be negligible. Furthermore, considering large-size antenna arrays are available at BSs, the short-term fading is ignored due to the channel hardening. The focus of this work is to mitigate interference from the coexisting 5G networks to the incumbent receiver in the shared satellite band. The joint mitigation of interference within the 5G cellular network and interference from the 5G-to-incumbent satellite receiver will be considered in our future work.}
% \begin{equation}
%     \label{capacity}
%     C_k=\sum_{m=1}^M\sum_{n=1}^{N} \sum_{u=1}^{F_{k,n}^{(m)}} z_{k,n}^{(m)} C_{k,m,n}^{(u)}.
% \end{equation}

% The resource optimization problem to dynamically control the BSs' RF parameters is formulated as
% \begin{equation}
% 	\label{optimization}
% 	\begin{split}
% 		\text{P0:} & \max_{\substack{ \bm{\nu} \in \{0,1\}, \\ \bm{z} \in \{0,1\}, \mathbf{P}}}  (1-w)\sum_{k=1}^K \nu_k C_k+ w\sum_{k=1}^K \sum_{m=1}^M\sum_{n=1}^{N} \nu_k z_{k,n}^{(m)} F_{k,n}^{(m)}\\
% 			& \text{s.t.} \begin{cases}
% 					&\hspace*{-0.3cm}  \text{C1:}~ \hspace{0.2cm} \sum_{k=1}^K \nu_k I_k \leq I_{th}\\
%                         &\hspace*{-0.3cm}  \text{C2:}~ \hspace{0.2cm} \min_{u \in \mathcal{U}_k} C_{k,n}^{(u)} \geq R_{th}, \forall k  \in \mathcal{K}\\
%                         &\hspace*{-0.3cm} \text{C3:}~ P_k \leq P_{max}, \forall k \in \mathcal{K}\\
%                         %&\hspace*{-0.3cm}  \text{C4:}~ r_e \geq r_{min}\\
%                         &\hspace*{-0.3cm} \text{C4:} \sum_{n=1}^N z_{k,n}^{(m)}=1, \forall m,k\\
%                         & \hspace*{-0.3cm} \text{C5:}~ v_k=0, \hspace{0.2cm} \text{if}  \hspace{0.2cm} d_{k,SAT} \leq r_{e}, \forall k \in \mathcal{K}.
%              \end{cases}
% 	\end{split}
% \end{equation}
% In $\text{P0}$, the objective function  maximizes a weighted sum of the achievable downlink capacity of the 5G cellular network and the number of UEs supported by it. Here, $w \in (0,1)$ as a predefined weight factor. The considered objective function maximizes the utilization of the shared satellite band for the coexisting 5G cellular network while ensuring fairness.  
% In $\text{P0}$, constraint $\text{C1}$ implies that the total interference introduced by the coexisting  5G cellular network to the incumbent receiver must be smaller than a predefined threshold $I_{th}$; constraint $\text{C2}$ implies a rate quality-of-service (QoS) constraint for the coexisting cellular networks'  UEs with $C_{th}$ as the minimum required downlink data rate and $\mathcal{U}_k$ as the set of all UEs supported by  the $k$-th BS; constraint $\text{C3}$ implies that the transmitted power from each BS must be smaller than a regulator defined maximum transmit power limit, $P_{max}$, over the shared satellite band; constraint $\text{C4}$ implies that only one codebook vector is loaded at each sub-array of a BS; constraint $\text{C5}$ implies that any BS within the regulator defined exclusion zone (of radius $r_e$) around the incumbent receiver must not be operative in the shared satellite band.

% \begin{proposition}
%     $\text{P0}$ is an NP-hard optimization problem.
% \end{proposition}

% \proof The proof is provided in Appendix A.

% Since $\text{P0}$ is an NP-hard optimization problem, it cannot be solved in polynomial time. In the next sub-section, we propose a heuristic algorithm to solve $\text{P0}$ in polynomial time.

% \subsubsection{Proposed Algorithm to Solve $\text{P0}$}
%  To efficiently solve $\text{P0}$, we decompose the overall optimization into three sub-tasks, namely, (T1) active beam selection, (T2) active BS selection, and (T3) transmit power control.  The overall algorithm to solve $\text{P0}$ by iteratively solving these sub-tasks is summarized as Algorithm \ref{Algorithm1}. A detailed description of the sub-tasks is provided as follows.
 
% % it into three sub-problems, namely, (1) active beam selection problem, (2) transmit power control %problem, and (3) BS activation problem. In what follows, we first near-optimally solve these sub-problems and subsequently, develop the overall algorithm to solve $\text{P0}$
 
%  %A sub-optimal yet efficient solution to $\text{P0}$ can be obtained by alternately solving the following  three sub-problems, namely, (1) active beam selection problem, (2) transmit power control problem, and (3) BS activation problem.  In what follows, we first develop suitable algorithms for these sub-problems and subsequently, develop the overall algorithm to solve $\text{P0}$.         
% \setlength{\textfloatsep}{0pt}
% \begin{algorithm}
% 	\caption{\textbf{Context-Aware Automated BS Control Algorithm for Spectrum Coexistence in Satellite Band}}
% 	\label{Algorithm1}
% 	\begin{algorithmic}[1]
%  \footnotesize
%      \State \textbf{Input:} Contextual factors (weather, RF propagation model, 5G deployment information (location and heights of BSs and buildings in the environment)); system variables (incumbent receiver's location and pointing angle); interference threshold $I_{th}$ and regulator defined exclusion zone's radius $r_e$; maximum number of iterations $T_{max}$.

% \State Determine the minimum transmit power $P_{min}^{(k)}$ for the $k$-th BS, $\forall k \in \mathcal{K}$

% \State Determine the set of non-operational BSs  $\mathcal{K}_{off}=\{k \in \mathcal{K}| d_{k,SAT} \leq r_e \cup  P_{min}^{(k)} >P_{max} \}$. Assign $\nu_k=0$ and $z_{k,m}^{(n)}=0$, and $P_k=0$, $\forall k \in \mathcal{K}_{off}, m \in \{1,2, \cdots, M\}, n \in \mathcal{N}$.

% \State \textbf{Initialize:} The set of operational BSs $\mathcal{K}_o= \mathcal{K} \setminus \mathcal{K}_{off}$;  $\mathcal{N}_k= \{1,2,\cdots, M\}$, $D_k=0$, $\nu_k=0$, $z_{k,m}^{(n)}=0$, $P_k=P_{min}^{(k)}$, $\forall k \in \mathcal{K}_o, m \in \{1,2, \cdots, M\}, n \in \mathcal{N}$; $\mathcal{S}=\{k \in \mathcal{K}_o |D_k < M \}$; $I_{agg}=0$.

% \State  Calculate $\rho_{k,m,n}=\frac{ (1-w)\sum_{u=1}^{F_{k,n}^{(m)}} C_{k,m,n}^{(u)} +w F_{k,n}^{(m)}}{I_{k,m,n}}$, $\forall k \in \mathcal{K}_o, m \in \{1,2, \cdots, M\}, n \in \mathcal{N}$.

% \Repeat 
%     \State Find $(k^*, m^*, n^*)=\arg \max_{\substack{k \in \mathcal{S},\\ m \in \mathcal{N}_k,\\ n \in \mathcal{N}}} \rho_{k,m,n}$.
    
%     \State Assign $z_{k^*,m^*}^{(n^*)}=1$. Update $\mathcal{N}_{k^*} \leftarrow \mathcal{N}_{k^*}  \setminus \{m^*\}$, $D_{k^*}=D_{k^*}+1$, and $\mathcal{S}=\{k \in \mathcal{K}_o |D_k < M \}$.

% %    \State Deactivate the $n^*$-th beam at the  $k^*$-th BS and update the  $k^*$-th BS's  active beam set by $\mathcal{N}_{k^*}^{(a)} \leftarrow \mathcal{N}_{k^*}^{(a)} \setminus \{n^*\}$ 

%  \State Update the aggregated interference $I_{agg} \leftarrow I_{agg}+10^{\frac{I_{k^*,m^*, n^*}}{10}}$.

%  \Until{$I_{agg} \leq I_{th}$ or $\mathcal{S}=\varnothing$} 

% \State Determine $\mathcal{K}_a=\{ k \in \mathcal{K}_o | D_k > 0 \}$. Assign $\nu_k=1$, $\forall k \in \mathcal{K}_a$.


% \State Assign $P_k=0, \forall k \in \mathcal{K}_o \setminus \mathcal{K}_a$. Solve $\text{P4}$ using off-the-shelf linear programming solver and update transmit power allocation $P_k, \forall k \in \mathcal{K}_a$.

% %\State Calculate the objective function value $\text{obj}(t)=(1-w)\sum_{k=1}^K \nu_k C_k+ w\sum_{k=1}^K \sum_{m=1}^M\sum_{n=1}^{N} \nu_k z_{k,n}^{(m)} F_{k,n}^{(m)}$. 

% %\State Assign $\mathcal{K}_o \leftarrow \mathcal{K}_a$ and $\overline{P}_k \leftarrow P_k, \forall k \in \mathcal{K}$; $t=t+1$. 

% %\Until {$|\text{obj}(t+1)-\text{obj}(t)| \leq \epsilon$ or $t>T_{max}$}

% \State \textbf{Output:} $\{\nu_k\}$, $\{z_{k,n}^{(m)}\}$, $\{P_k\}$.
% \end{algorithmic}
% \end{algorithm}

% \paragraph{T1: Active Beam Selection}
% The objective of this sub-task is to select a suitable set active beams of the operational BSs while considering a fixed power allocation per BS. We denote $\mathcal{K}_o$ as the set of operational BSs. The active beam selection problem is therefore formulated as 
%  \begin{equation}
% 	\label{optimization}
% 	\begin{split}
% 		\text{P1:} & \max_{\bm{z} \in \{0,1\}}  \sum_{k \in \mathcal{K}_o} \sum_{m=1}^M \sum_{n=1}^{N} z_{k,n}^{(m)} \left((1-w)\sum_{u=1}^{F_{k,n}^{(m)}} C_{k,m,n}^{(u)} +w F_{k,n}^{(m)}\right) \\
%   	 &  \text{s.t.} 
%              \begin{cases}
%   			   & \sum_{k \in \mathcal{K}_o} \sum_{m=1}^M \sum_{n=1}^{N} z_{k,n}^{(m)} 10^{\frac{I_{k,m,n}}{10}} \leq I_{th}\\
%                      &  \sum_{n=1}^N z_{k,n}^{(m)}=1, \forall m \in \{1,2, \cdots, M\}, k  \in \mathcal{K}.
%   			 \end{cases}
% 	\end{split}
% \end{equation}

% %$\text{P1}$ determines the optimal set of beams that each operational BS can keep active in order to maximize the utilization of the shared band under the assumption that each BS transmits at the minimum required power level.

% $\text{P1}$ aims to select a suitable codebook vector for the sub-arrays of each operational BS such that the spectrum utilization is maximized while keeping the aggregated interference at the incumbent receiver less than the threshold level. Although $\text{P1}$ is equivalent to a multiple-choice Knapsack problem, it can be effectively solved using a greedy approach. Steps 4-10 of Algorithm \ref{Algorithm1} outline the proposed (greedy) approach of solving $\text{P1}$. Here, $\mathcal{N}_k$ denotes the set inactive sub-arrays of the $k$-th BS\footnote{A sub-array is inactive if no codebook is selected for it and thereby, it does not create any beam}; $D_k$ denotes number of active sub-arrays of the $k$-th BS; and $\mathcal{S}$ denotes the set of operational BSs having less than $M$ active sub-arrays.   At Step 4 of Algorithm \ref{Algorithm1}, we initialize $\{\mathcal{N}_k\}$, $\{D_k\}$, $\mathcal{S}$, and optimization variables. More precisely, we consider that all the sub-arrays are inactive and thereby,  the aggregated interference is zero. The essence of our proposed approach is to sequentially activate the best combination of BS, sub-array, and beam vector. To this end, in Step 5 of Algorithm \ref{Algorithm1},   we calculate a  priority score, denoted by $\{\rho_{k,m,n}\}$, which provides a ratio of the  overall band utilization to interference power generated by the beam created by loading the $n$-th codebook vector to the $m$-th sub-array of the $k$-th BS, $\forall k,m,n$. In Steps 7-9, we iteratively activate the best beam with the highest $\{\rho_{k,m,n}\}$ score,  update $\{\mathcal{N}_k\}$, $\{D_k\}$, $\mathcal{S}$, and update the aggregated interference $I_{agg}$. This procedure is iteratively repeated until $I_{agg} \leq I_{th}$ or the $\mathcal{S}$ set is empty.

% \paragraph{T2: Active BS Selection}
% In this sub-task, we aim to select a suitable set of BSs from a given set of operational BSs, $\mathcal{K}_o$, considering that the set of active beams and transmit power of these BSs are known. The active BS selection problem is formulated as
% \begin{equation}
% 	\label{optimization}
% 	\begin{split}
% 		\text{P2:} & \max_{\bm{\nu} \in \{0,1\}}  \sum_{k \in \mathcal{K}_o} \nu_k \Delta_k\\
%   	&\hspace{-0.8cm} \text{s.t.}~ 
% 		\sum_{k \in \mathcal{K}_o} \nu_k \sum_{m=1}^M \sum_{n \in \mathcal{N}}  z_{k,n}^{(m)} 10^{\frac{I_{k,m,n}}{10}} \leq I_{th}\\
%       %& \hspace*{-0.3cm} ~ v_k=0, \hspace{0.2cm} \text{if}  \hspace{0.2cm} d_{k,SAT} \leq r_{e}, \forall k \in \mathcal{K}.
% 	\end{split}
% \end{equation}
% where 
% \begin{equation}
%     \label{Delta}
%     \begin{split}
%         \Delta_k=& (1-w)\sum_{m=1}^{M} \sum_{n=1}^{N} \sum_{u=1}^{F_{k,n}^{(m)}} z_{k,n}^{(m)}C_{k,m,n}\\
%         &+w\sum_{m=1}^{M} \sum_{n=1}^{N} z_{k,n}^{(m)} F_{k,n}^{(m)}.
%     \end{split}
% \end{equation}

% $\text{P2}$ is equivalent to a $0/1$-Knapsack problem, and consequently, similar to $\text{P1}$,  an iterative greedy approach can be employed to efficiently solve $\text{P2}$. Note that the task T1 selects active beams for the BSs in $\mathcal{K}_o$ set  in such a way so that the aggregated interference constraint is satisfied for all the BSs in the $\mathcal{K}_a \subset \mathcal{K}_o$ set. Here, $\mathcal{K}_a=\{k \in \mathcal{K}_o| D_k > 0\}$ denotes the set of BSs having one or more active sub-arrays. Meanwhile, since all the sub-arrays of each BS in the  $\mathcal{K}_o \setminus \mathcal{K}_a $ set are inactive, these BSs cannot be operational in the shared band. At the same time, we can also justify that the objective function value of $\text{P2}$ is strictly decreased when only a sub-set of BSs in the  $\mathcal{K}_a$ set remain operational. Therefore, $\mathcal{K}_a$  is the optimal set of operational BSs, and consequently, the optimal solution to $\text{P2}$ is obtained as $\nu_k=1$, $\forall k \in \mathcal{K}_a$ and $\nu_k=0$, $\forall k \in \mathcal{K}_o \setminus \mathcal{K}_a$.


% \paragraph{T3: Transmit Power Control Problem}
% %Algorithm \ref{Alg_Beam} provides the optimal set of beams for the operational BSs in the shared satellite band. However, a conservative spectrum sharing scenario is considered by limiting each active BS's transmit power to  the minimum required power level. In practice, depending on the several contextual factors, such as weather and deployment scenarios, a BS can transmit higher power than the minimum power level without causing harmful interference at the incumbent satellite receiver. 
% Here, we  aim to optimize the transmit power of the operational BSs in order to maximize the downlink capacity of the 5G cellular network while considering that the set of active beams per BS is known. The transmit power control problem is formulated as
% \begin{equation}
% 	\label{optimization}
% 	\begin{split}
% 		\text{P3:}\hspace{0.2cm} & \max_ {\mathbf{P}}  \sum_{k \in \mathcal{K}_o} \sum_{m=1}^M \sum_{n=1}^N \sum_{u=1}^{F_{k,n}^{(m)}} \nu_k z_{k,n}^{(m)} C_{k,m,n}^{(u)} \\
%   		&\hspace{-0.8cm} \text{s.t.} \begin{cases}
% 					& \sum_{k \in \mathcal{K}_o} \sum_{m=1}^M \sum_{n \in \mathcal{N}} \nu_k z_{k,n}^{(m)} P_k 10^{\frac{\overline{G}_{k,m,n}}{10}} \leq I_{th}\\
%                    & P_{min}^{(k)} \leq P_k \leq P_{max}, \forall k \in \mathcal{K}\\
%              \end{cases}
%      	\end{split}
% \end{equation}
% where $\overline{G}_{k,m,n}=G_{5G}^{(k)}\left(\theta_{n,int}, \phi_{n,int}\right)+ G_{SAT}(\phi_{k, SAT})-\text{PL}(d_{k,SAT})-10\log_{10}(M)$ denotes the effective interference channel gain (in dB) between the $n$-th beam transmitted from the $k$-th BS's $m$-th sub-array and the incumbent receiver, and $P_{min}^{(k)}$ denotes the minimum required transmit power from the $k$-th BS,  $\forall k \in \mathcal{K}_o$. From constraint $\text{C2}$, we obtain $P_{min}^{(k)}=\left(2^{R_{th}}-1 \right) \frac{NP}{\min_{u \in \mathcal{U}_k}10^{\frac{\overline{H}_{k,n}^{(u)}}{10}}}$, where $\overline{H}_{k,n}^{(u)}= H^{(n)}\left(\Theta_{n}, \Theta_u\right)-\text{PL}(d_{k,u})-10\log_{10}(M)$. In the absence of aggregate interference constraint, the optimal solution to $\text{P3}$ is always obtained as $P_k=P_{max}$, $\forall k \in \mathcal{K}_a$ and $P_k=0$, $\forall k \in\mathcal{K}_0 \setminus \mathcal{K}_a$. This is intuitive since  a noise-limited scenario is considered for the coexisting cellular network, and hence, the overall downlink capacity of the  cellular network is always improved with the increase of power transmitted from the BSs. Inspired by such a observation, a suitable solution to $\text{P3}$ can be obtained by maximizing the total transmitted power from all the active BSs subject to the aggregate interference and power limit constraints. Such an optimization problem is formulated as
% \begin{equation}
% 	\label{optimization}
% 	\begin{split}
% 		\text{P4:}\hspace{0.2cm} & \max_{\mathbf{P}}  \sum_{k \in \mathcal{K}_a} \Omega_k P_k \\
%   		&\hspace{-0.8cm} \text{s.t.} \begin{cases}
% 					& \sum_{k \in \mathcal{K}_a} P_k \Lambda_k  \leq I_{th}\\
%                    & P_{min}^{(k)} \leq P_k \leq P_{max}, \forall k \in \mathcal{K}_a\\
%              \end{cases}
%      	\end{split}
% \end{equation}
% where $\Lambda_k=\sum_{m=1}^M \sum_{n \in \mathcal{N}} z_{k,n}^{(m)} 10^{\frac{\overline{G}_{k,m,n}}{10}}$,  and $\Omega_k=\frac{\sum_{m=1}^M \sum_{n=1}^N z_{k,n}^{(m)} F_{k,n}^{(m)}}{\sum_{k \in \mathcal{K}_a} \sum_{m=1}^M \sum_{n=1}^N z_{k,n}^{(m)} F_{k,n}^{(m)}}$, $\forall k \in \mathcal{K}_a$. Here, $\Omega_k$ is a weight factor representing the importance of increasing transmit power of an active BS. Particularly, if an active BS has activates large number of beams and supports a high number of UEs, it has more importance in terms of increasing its transmit power compared to the BSs with few active beams. Thus, solving $\text{P4}$ allows to increase and decrease the transmit power of more important and less important BSs while satisfying the aggregate interference threshold.  Note that since $\text{P4}$ is a linear programming problem,  it can readily be solved using off-the-shelf solvers.


% %and it has at least only one feasible solution,  i.e.,  $P_k=\overline{P}_k, \forall k \in \mathcal{K}_a$. Accordingly, $\text{P4}$ must have an optimal solution, which can readily be obtained using off-the-shelf solvers. The overall transmit power control algorithm is summarized in Algorithm \ref{Alg_Power}.  




% %This is because Algorithm \ref{Alg_Power} determines transmit power of the BSs in $\mathcal{K}_a$ set 

% %The overall steps to solve $\text{P4}$ are summarized as Algorithm \ref{Alg_BS}. In Algorithm \ref{Alg_BS}, $\mathcal{K}_a$ and $\mathcal{K}_{temp}$ represents an optimal set of operational BSs and a set of all BSs having non-zero transmit power, respectively. We initialize  $\mathcal{K}_a$ as an empty set and evaluate the aggregate interference, $I_{agg}$, for all the BSs belong the $\mathcal{K}_{temp}$ set (Step 2 and 3).  If $I_{agg} \leq I_{th}$,  all the non-zero power BSs can reamine active and hence, Algorithm \ref{Alg_Beam} is terminated (Step 5). Otherwise, we first calculate a priority score for each BS, denoted by \{$\eta_k\}$,  where $\eta_k$ provides a ratio between the overall band utilization factor (i.e., sum of downlink rate and number of supported UEs) and the total generated interference from the $k$-th BS to the incumbent receiver (Step 7).  Subsequently, we iteratively pick up  the BS  having the largest  priority scores from the  $\mathcal{K}_{temp}$ set and add it  to the $\mathcal{K}_a$ set (Steps 9-12). This procedure is continued as long as the total interference from the BSs  in the $\mathcal{K}_a$ set, denoted by $I_T(\mathcal{K}_a)$, remains smaller than or equal to $I_{th}$.
% %   \setlength{\textfloatsep}{0pt}
% %\begin{algorithm}
% %	\caption{\textbf{Operational BS Selection Algorithm}}
% %	\label{Alg_BS}
% %	\begin{algorithmic}[1]
% %\State \textbf{Input:} Given set of BSs $\mathcal{K}_o$; set of active beams per BS, $\mathcal{N}_k^{(a)}$, transmit power allocation $\{P_k^*\}$, \# supported UEs per beam, $F_{k,n}$, $\forall k \in \mathcal{K}_o, n \in \mathcal{N}_k$; interference threshold, $I_{th}$.

% %\State \textbf{Initialize:} $\mathcal{K}_{temp}=\{k \in \mathcal{K}_o| P_k^* \neq 0\}$, $\mathcal{K}_a= \varnothing$, and $I_T(\mathcal{K}_a)=0$.

% %\State Calculate $I_{k,n}$ by plugging $P_k^*$ to \eqref{interfernece}, $\forall k \in \mathcal{K}_{temp}, n \in \mathcal{N}_k^{(a)}$. Calculate the aggregated interference $I_{agg}=\sum_{k \in \mathcal{K}_{temp}} \sum_{n \in \mathcal{N}_k^{(a)}} 10^{\frac{I_{k,n}}{10}}$.

% %\If {$I_{agg} \leq I_{th}$}

%   % \State Return $\mathcal{K}_a=\mathcal{K}_{temp}$; Break

%  %  \Else 

% %\State Calculate $\eta_{k}=\frac{  \sum_{n \in \mathcal{N}_k^{(a)}} (1-w)\sum_{u=1}^{F_{k,n}} C_{k,n}^{(u)}+w F_{k,n}}{\sum_{n \in \mathcal{N}_k^{(a)}} 10^{\frac{I_{k,n} \left(P_k^{*}\right)}{10}}}$, $\forall k \in \mathcal{K}_{temp}$.
     
%    %\While {$I_T(\mathcal{K}_a) \leq I_{th}$}
%    %\State Find $k^*=\arg \max_{k \in \mathcal{K}_{temp}} \eta_k$.

%   % \State $\mathcal{K}_a \leftarrow \mathcal{K}_a \cup \{k^*\}$ and $\mathcal{K}_{temp} \leftarrow  \mathcal{K}_{temp} \leftarrow  \mathcal{K}_{temp} \setminus \{k^*\}$

%  %  \State Update the total interference from BSs in the $\mathcal{K}_a$ set:  $I_T(\mathcal{K}_a) \leftarrow I_T(\mathcal{K}_a)+\sum_{n \in \mathcal{N}_{k^*}^{(a)}}  10^{\frac{I_{k^*,n} \left(P_k^{*}\right)}{10}}$.

% %\EndWhile
% %\EndIf

% %\State \textbf{Output:} The updated set of operational BSs in the shared satellite band, $\mathcal{K}_a$.

% %\end{algorithmic}
% %\end{algorithm}


% \paragraph{Overall Algorithm}
% Algorithm \ref{Algorithm1}  solves problem P0 using the following steps. In Step 2, we determine the minimum required transmit power for each BS. In Step 3, we identify the set of BSs, $\mathcal{K}_{off}$, that must be non-operational in the shared satellite band. A BS is non-operational in the satellite band if either one of following two conditions are satisfied: (1) the BS is within the regulator defied exclusion zone around the incumbent satellite receiver or (2) it requires a minimum power level exceeding the maximum allowed transmit power limit in the shared band\footnote{This condition arises when the UEs connected with the BS exhibit severe path loss in the band of interest, making it impossible to satisfy their minimum data rate requirements with the given transmit power limit. Consequently, these BSs  cannot be operational in the shared satellite band.}. In Step 4, we initialize the set of operational BSs and select the minimum transmit power level for each operational BS. In  Steps 5-12, the set of active beams directions of operational BSs, set of active BSs, and transmit power allocations of active BSs are  updated by sequentially executing the aforementioned sub-tasks T1-T3, respectively. Step 13 of Algorithm \ref{Algorithm1} provides the solution to problem $\text{P0}$.
% %In Step 15, the objective function value of $\text{P0}$ is calculated for the obtained RF parameters.  The aforementioned iteration is continued till a converged objective function is obtained or the maximum number of iterations is reached. If a converged solution is not found within the specified number of iterations, the output of Algorithm \ref{Algorithm1} is determined as the set of operational BSs along with their corresponding RF parameters that yield the maximum objective value calculated in Step 15. 
% %This ensures that Algorithm \ref{Algorithm1} must provide a feasible solution even if the convergence is not achieved .

% \begin{proposition}
%     The worst-case time complexity of Algorithm \ref{Algorithm1} is $\mathcal{O}\left(MKN \log MKN + K^{3.5}\log(1/\epsilon) \right)$, where $\epsilon \in (0,1)$ is the predefined error-tolerance factor.
% \end{proposition}

%  \proof The time complexity of Algorithm \ref{Algorithm1} is dominated by the complexity of  executing Steps 5-12. The time complexity of executing Steps 5 is $\mathcal{O}(MKN)$. Steps 6-10 present a loop for selecting active set of beam of a given set of operational BSs. In particular,  Steps 7, 8, and 9 are iteratively repeated within this inner loop, whose time complexity is  $\mathcal{O(MKN \log MKN)}$, $\mathcal{O}(1)$, and $\mathcal{O}(1)$, respectively. Accordingly, the  overall time complexity of executing Steps 6-10 is obtained as $\mathcal{O}\left(2+ MKN\log MKN\right) \approx \mathcal{O}\left(MKNN\log MKN\right)$. Step 11 is used for updating the set of active BSs, whose time complexity is $\mathcal{O}(1)$. Step 12 is used to update the transmit power allocation by solving  a linear programming problem $\text{P4}$ with at most $K$ variables. Considering that a interior-point method is used to solve $\text{P4}$, the time complexity of Step 12 is obtained as $\mathcal{O}\left(K^{3.5}\log(1/\epsilon)\right)$. Hence, the worst-case time complexity of Algorithm \ref{Algorithm1} is obtained as $\mathcal{O}\left(MKN+MKN \log MKN+ K^{3.5}\log(1/\epsilon) \right) \approx \mathcal{O}\left(MKN \log MKN + K^{3.5}\log(1/\epsilon) \right)$. \QED
 
 
% \textit{\textbf{Remark 1}}:  There is a notable distinction between the proposed Algorithm \ref{Algorithm1} and the conventional exclusion zone-based spectrum sharing approach. Conventionally, a deterministic approach is adopted, where only the BSs located outside a predefined exclusion zone are activated without taking any contextual factors into account. In contrast, Algorithm \ref{Algorithm1} takes a dynamic approach in determining the set  of operational BSs and their associated parameters, namely, the set of active beams and transmit power. More specifically, Algorithm \ref{Algorithm1} validates the suitability of the decision variables by plugging them into the realistic interference evaluation framework, and thereby,  takes different contextual factors  and system variables into account. This enables Algorithm \ref{Algorithm1} to activate more BSs and/or more beams per BS compared to the conventional exclusion zone-based BS activation policy without disrupting the operations of incumbent satellite receivers.







% \subsection{O-RAN Based Implementation}

% Here we need to describe two different things:

% \begin{itemize}
%     \item Spectrum sharing xAPP development based on the control algorithms

%     \item Collection of information (context and feedback) and providing control decisions to the BSs. All these things can be explained using a timing diagrams (Rob need to work on that)
% \end{itemize}

% The O-RAN framework was selected for implementation based on its suitability for incorporating context information, hosting the system model and algorithm, and future availability of the necessary RAN control mechanisms. The RAN Intelligent Controller (RIC) is designed to enable third-party algorithms to influence RAN behavior through policy changes and direct control of RAN parameters and decisions via a standardized interface. The Traffic Steering use case, an O-RAN Alliance standardized use case for mobility optimization, defines mechanisms for control of handover decisions based on learned strategies .(Cite?) Our implementation follows a similar approach. Figure \ref{fig_4} shows how O-RAN standardized components are utilized to implement core functions of the system. Context information (how did you implement the context acquisition unit? We can describe it as an entity within the SMO) is fed to the System Model via?. The System Model provides enrichment data to the algorithm... The near-realtime RIC hosts the Algorithm as an xApp. The E2 interface communicates control decisions to the network. 

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=0.95\linewidth, draft=false]{Figures/vt_12_ghz.png}
% 		\caption{Proposed context-aware BS control flow.}
% 		\label{fig_4}
% 	\end{center}
% \end{figure}

% \section{Performance Evaluation}

% \subsection{Description of Experimental Setup}
% \textcolor{blue}{We have to provide the information of the Blacksburg environment, similar to WCL paper. Additional information, such as code-book-based beamforming, the FSS receiver's pointing angle should be included.}

% For the experimental environment of the interference analysis in the coexistence of 5G terrestrial MBS, and FSS receiver at $12$ GHz satellite band, we consider a suburban area of Blacksburg City, Virginia having a population density of $2270$ per square mile \cite{RKFreport, popuden}. This realistic deployment scenario is set based on the real location of the FSS receiver which is at 1770 Forecast Drive in Blacksburg (37° 12' 9" North latitude and 80° 26' 4" West longitude), and the $33$ Global System for Mobile communication(GSM) MBSs within the $5000$m circular area of the FSS location leveraging the OpenCellID dataset. Each MBS operates on a $1000$m cellular coverage area divided into three sectors ($120^\circ$ each), accommodating $10$ randomly located UEs and a total of $12$ subarrays. For an accurate and site-specific pathloss analysis as discussed in Section IV, we incorporate 8644 building information: heights ($10$m to $40$m), shapes, polygons, and geolocation from OpenStreetMap via overpass-turbo. Furthermore, for the beamforming capabilities in Section IV, we consider $4\times4$ directional planner antenna array with $0.5\lambda$ element spacing and $64$ predefined beams in each subarray. Again, as per 3GPP, the specified nominal transmit power for an MBS is set at 38 dBm. Consequently, in our interference analysis for individual MBSs, we explore a power range from $-2$ dBm to $+2$ dBm relative to this nominal value of 38 dBm. Additionally, we consider various FSS pointing angles ($20^\circ$, $30^\circ$, $40^\circ$, and $50^\circ$), a down-tilt angle of $10^\circ$ suggested by \cite{RKFreport} and interference thresholds for sunny and rainy weather, we consider $-8.5$ dB and $-12$ dB \cite{RKFreport, SpaceXanalysis} for the analysis of aggregated interference to noise ratio (I/N) and achievable downlink capacity. To make it a context-aware analysis we consider normal and rainy weather using the weather-specific data of a particular day from the OpenWeatherMap. Moreover, our proposed algorithm aims to maximize the number of active MBSs while ensuring that interference levels remain below the acceptable thresholds for a particular weather to mitigate the harmful interference at the FSS receiver. This algorithm dynamically adjusts the parameters: power levels, antenna and beam configurations, angles of UEs, and MBSs with respect to the FSS receiver. Therefore, to accomplish the goal, we analyze the interference-to-noise ratio, achievable downlink capacity, and the number of active MBSs considering the FSS mobility within ($20^\circ$ to $50^\circ$), various sizes of antenna elements, and codebook beams, specifically the antenna configurations of $4$x$4$, $4$x$16$, and $16$x$16$ in both the horizontal and vertical directions.

% \subsection{Experiment Results: Interference Mitigation Performance}

% \begin{enumerate}

%     \item \textbf{Aggregate I/N variations for different pointing angles' of FSS receivers for proposed and exclusion zone-based BS on/off scheme at different weather conditions.}:
%     \setlength{\textfloatsep}{0pt}
%      \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={1cm 0cm 1cm 0cm},clip,width=9cm]{Figures/Sunny_I_N.pdf}
%     		\caption{Aggregate I/N Vs FSS Pointing Angles}
%     		\label{fig_3}
%     	\end{center}
%     \end{figure}
% Fig.\ref{fig_3} presents a statistical analysis of interference variations under different FSS pointing angles in normal atmospheric conditions. This bar plot also compares the aggregated I/N for the active MBSs outside an exclusion zone radius of $3000$m and for the active MBSs maintaining an interference threshold of $-15$dB with a reference baseline of \cite{12GHz_WCL}. It is observed that for a given FSS pointing angle, the aggregated I/N values for the operational MBSs derived from our proposed algorithm outperform the baseline values. Whereas, these values remain consistent across all the FSS elevation angles. The potential reason behind that in the simulation environment, the elevation angles used by the FSS receiver and the elevation angles employed in the optimization algorithm are identical. Hence the algorithm optimizes the parameters in such a way that the aggregate I/N always remains less than the threshold.
    
    
% \item  \textbf{Number of active MBSs for different pointing angles' of FSS receivers for proposed and exclusion zone-based BS on/off scheme at different weather conditions}: 
%  \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={0cm 0cm 2cm 0cm},clip,width=9cm]{Figures/Sunny_Active_BS.pdf}
%     		\caption{ Number of Active BS Vs FSS Pointing Angles}
%     		\label{fig_4}
%     	\end{center}
%     \end{figure}
% Fig.\ref{fig_4} shows the count of operational MBSs resulting from the BS control algorithm and the two baselines from \cite{12GHz_WCL}. We utilize a bar graph to represent the number of operational MBSs across various FSS elevation angles. Through the implementation of our BS control algorithm, we can operate a maximum of $19$ MBSs. This number exceeds the count of MBSs located outside the $3000$m exclusion zone and the count of active MBSs that adhere to an interference threshold of $-15$ dB which are counted as $8$ and $7$ respectively.

% \item \textbf{Achievable Downlink Capacity vs. FSS Elevation Angles for different weather}: 
%            \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={1cm 2cm 12cm 2.5cm},clip,width=9cm]{Figures/Sunny_cap.pdf}
%     		\caption{Achievable Downlink Capacity Vs FSS Pointing Angles}
%     		\label{fig_5}
%     	\end{center}
%     \end{figure}
% For a sunny day, we illustrated an analysis of aggregate downlink throughput for all the operational MBSs as a result of our heuristic algorithm in Fig.\ref{fig_5}. We present the bar graph as a comparison of our algorithm's performances with the benchmark schemes. Both the benchmark schemes and the proposed algorithm exhibit a trade-off between the number of active MBSs and achievable downlink throughput. Increasing the number of operational MBS through the BS control algorithm significantly enhances the overall achievable downlink throughput reaching almost $75000$ bps/Hz. However, the proposed algorithm allows the activation of the maximum number of MBSs, resulting in a higher aggregate capacity that surpasses the other two cases, which involve a lower number of active MBSs and a lower aggregate throughput. This emphasizes the efficacy of our heuristic algorithm in maximizing the network's capacity by leveraging a larger number of MBSs.

     

% \item \textbf{Aggregate I/N ratio for various antenna array sizes for proposed and exclusion zone-based BS on/off scheme in different weather conditions}: 
%     \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={0.5cm 0cm 0cm 0cm},clip,width=9cm]{Figures/Sunny_I_N_Antenna164.pdf}
%     		\caption{ Aggregate I/N Vs Antenna element sizes}
%     		\label{fig_6}
%     	\end{center}
%     \end{figure}
% Fig.\ref{fig_6} depicts the variations in interference levels across different antenna sizes $4$x$4$, $4$x$16$, and $16$x$16$ in both the horizontal and vertical directions, under sunny weather conditions. We consider a barplot to showcase our interference-to-noise (I/N) analysis for various antenna sizes, comparing them with established baselines such as the exclusion zone and the -15dB threshold method as introduced in \cite{12GHz_WCL}. These graphs clearly indicate that our proposed algorithm consistently surpasses the baseline methods in terms of the aggregate I/N analysis for 5G MBSs' operation across all antenna patterns.


% % Exclusion zone-based BS turn on/off scheme, and criteria II-IV of WCL paper.  We also need to show a table similar to WCL how many BSs can be active by our proposed and benchmark schemes. We want to show our proposed scheme can work even with a small exclusion zone's radius and can also adapt to the weather conditions. 

% \item \textbf{Number of active MBSs considering various antenna element sizes for proposed and exclusion zone-based BS on/off scheme at different weather conditions.}: 
% \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={0.5cm 0cm 0cm 0cm},clip,width=9cm]{Figures/Sunny_active_bs_Antenna164.pdf}
%     		\caption{ Number of Active MBSs Vs Antenna element sizes}
%     		\label{fig_7}
%     	\end{center}
%     \end{figure}
    
% Under typical atmospheric conditions, Fig.\ref{fig_7}  presents a graphical depiction of the count of operational MBSs, derived from the BS control algorithm alongside the two baseline methods from \cite{12GHz_WCL}. We employed a bar graph to effectively illustrate the number of operational MBSs across previously discussed diverse antenna element sizes and our observation reveals that the proposed method consistently enables the activation of the max number of MBSs when compared to the baselines.  However, the trade-off between increasing antenna element sizes and the maximum number of operational MBSs underscores the impact of antenna size on MBS operations as by increasing the antenna element size we can get a highly directional beam which increases the 5G MBS antenna gain.


% \item \textbf{Achievable Downlink Capacity analysis in different antenna array sizes for proposed and exclusion zone-based BS on/off scheme in different weather conditions}:

%  \begin{figure}
%     	\begin{center}
%     	\includegraphics[trim={0cm 0cm 2cm 0cm},clip,width=9cm]{Figures/Sunny_cap_Antenna164.pdf}
%     		\caption{Achievable Downlink Capacity Vs Antenna element sizes}
%     		\label{fig_8}
%     	\end{center}
%     \end{figure}

% In Fig.\ref{fig_8}, the bar plot provides a statistical analysis of the aggregate downlink capacity for all the operational MBSs for three distinctive antenna array sizes on a sunny day. Our findings show that, since we are able to maximize the number of operational MBSs through our proposed method, the overall throughput is also maximized, outperforming the benchmarks. This relationship holds true when considering the proportional connection between the increasing antenna array sizes and the growing number of active MBSs. Hence, the achievable aggregate downlink capacity reaches its peak when utilizing the maximum array size for all scenarios of MBS operations. This underscores the effectiveness of our heuristic algorithm's performance in the maximum array size to increase the network's throughput by employing a larger number of MBSs. The potential reason behind that with the increasing number of antenna sizes we can get relatively shaper and highly directional beams which helps to enhance the SNR and eventually the total capacity of the system. 
% \end{enumerate}



% \subsection{Experimental Results: O-RAN Specific Performance}



% \section{Conclusion}


% \appendices

% \section{}
% If a special case of $\text{P0}$, obtained by either fixing certain variables and/or relaxing certain constraints, remain NP-hard, then $\text{P0}$ must be NP-hard. To this end, we consider that the transmit power of the BSs are predetermined. Accordingly, $\text{P0}$ is reduced to the joint optimization of selecting operational BSs in the shard satellite band and set of active beams per BS. Using two different cases, we can prove that such a reduced problem is NP-hard.

% \begin{itemize}
% \item We first assume that the set of active beams per BS, i.e, $\{z_{k,n}^{(m)}\}$, is given. 
% In this context, $\text{P0}$ can be expressed as
% 	\begin{equation}
% 		\label{optimization_1}
% 		\begin{split}
% 			& \max_{ \mathbf{\bm{\nu}} \in \{0,1\}} \sum_{k \in \mathcal{K}'} \nu_k C_k\\
% 			&\hspace{-0.8cm} \text{s.t.} \hspace{0.2cm} \sum_{k \in \mathcal{K}'} \nu_k I_k \leq I_{th}\\
% 			\end{split}
% 	\end{equation}
%  where $\mathcal{K}'=\{ k \in \mathcal{K}| d_{k, FSS} \leq r_e\}$. Eq. \eqref{optimization_1} is a 0-1 Knapsack problem with $\{C_k\}$ as the value per item, $\{I_k\}$ is the weight per item, and $I_{th}$ is the bound of total weight of the selected items. Since 0-1 Knapsack problem is a classic NP-hard problem, \eqref{optimization_1} is also NP-hard.

% \item Next, we assume that the set of operational MBSs is given such $\nu_k=1$ if $k \in \mathcal{K}'$ and $\nu_k=0$ otherwise.  Accordingly, $\text{P0}$ is reduced as 
% \begin{equation}
% 		\label{optimization_2}
% 	\begin{split}
% 		& \max_{\mathbf{\bm{z}} \in \{0,1\}} \sum_{k=1}^{K'} \sum_{m=1}^M \sum_{n=1}^{N} z_{k,n}^{(m)} \Psi_{k,n}^{(m)}\\
% 		& \hspace{-0.8cm} \text{s.t.}  \hspace{0.2cm} \sum_{k=1}^{K'} \sum_{m=1}^M \sum_{n=1}^{N}  z_{k,n}^{(m)} 10^{\frac{I_{k,m,n}}{10}}  \leq I_{th}\\
%    &  \sum_{n=1}^N z_{k,n}^{(m)}=1, \forall m \in \{1,2, \cdots, M\}, k  \in \mathcal{K}'.
%   	\end{split}
% \end{equation}
% where $\Psi_{k,n}^{(m)}=(1-w)\sum_{u=1}^{F_{k,n}^{(m)}} C_{k,m,n}^{(u)} +w F_{k,n}^{(m)}$. Eq. \eqref{optimization_1} is equivalent to a multiple-choice Knapsack problem, which is a classic NP-hard problem. Hence, \eqref{optimization_1} is also an NP-hard problem.
% \end{itemize}

% Since both \eqref{optimization_1} and \eqref{optimization_2} are individually NP-hard,  the special case of $\text{P0}$ obtained by fixing the BSs' transmit power is also NP-hard. This implies that $\text{P0}$ must be an NP-hard optimization problem. \QED 


    
% % \setlength{\textfloatsep}{0pt}
% % \begin{algorithm}
% % 	\caption{\textbf{ Active Beam Set Selection Algorithm}}
% % 	\label{Alg_Beam}
% % 	\begin{algorithmic}[1]
% % \State \textbf{Input:} Set of operational BSs $\mathcal{K}_o$; fixed transmit power, $\overline{P}_k$, set of beams per BS, $\mathcal{N}_k$, and \# supported UEs per beam, $F_{k,n}$, $\forall k \in \mathcal{K}_o, n \in \mathcal{N}_k$; interference threshold, $I_{th}$.

% % \State \textbf{Initialize:} $\mathcal{N}_k^{(a)}=\mathcal{N}_k$, $\forall k \in \mathcal{K}_o$.

% % \State Calculate $I_{k,n}$ by plugging $\overline{P}_k$ to \eqref{interfernece}, $\forall k \in \mathcal{K}_0, n \in \mathcal{N}_k^{(a)}$. Calculate the aggregated interference $I_{agg}=\sum_{k \in \mathcal{K}_o} \sum_{n \in \mathcal{N}_k^{(a)}} 10^{\frac{I_{k,n}}{10}}$. 

% % \If {$I_{agg} \leq I_{th}$}

% %    \State Return $\mathcal{N}_k^{(a)}$; Break

% %    \Else 

% %          \State Calculate $\rho_{k,n}=\frac{ 10^{\frac{I_{k,n}}{10}}}{(1-w)\sum_{u=1}^{F_{k,n}} C_{k,n}^{(u)} +w F_{k,n}}$, $\forall k \in \mathcal{K}_o$ and $\forall n \in \mathcal{N}_k$.

% %    \Repeat 
% %    \State Find $(k^*, n^*)=\arg \max_{k \in \mathcal{K}_o, n \in \mathcal{N}_k^{(a)} } \rho_{k,n}$.

% %    \State Deactivate the $n^*$-th beam at the  $k^*$-th BS and update the  $k^*$-th BS's  active beam set by $\mathcal{N}_{k^*}^{(a)} \leftarrow \mathcal{N}_{k^*}^{(a)} \setminus \{n^*\}$ 

% %    \State Update the aggregated interference $I_{agg} \leftarrow I_{agg}-10^{\frac{I_{k^*,n^*}}{10}}$.

% % \Until{$I_{agg} \leq I_{th}$}
% % \EndIf

% % \State \textbf{Output:} The set of active beams of the $k$-th BS, $\mathcal{N}_k^{(a)}$, $\forall k \in \mathcal{K}_o$.

% % \end{algorithmic}
% % \end{algorithm}

% % \setlength{\textfloatsep}{0pt}
% % \begin{algorithm}
% % 	\caption{\textbf{Transmit Power Control Algorithm}}
% % 	\label{Alg_Power}
% % 	\begin{algorithmic}[1]
% % \State \textbf{Input:} Set of operational BSs $\mathcal{K}_o$; set of active beams per BS, $\mathcal{N}_k^{(a)}$; interference threshold, $I_{th}$.

% % \State $\exists k \in \mathcal{K}_o$ and $\mathcal{N}_k^{(a)}=\varnothing$, set $P_k=0$. Determine $\mathcal{K}_o'=\{k \in \mathcal{K}_o| \mathcal{N}_k^{(a)} \neq \varnothing\}$.

% % \State Find the optimal transmit power of all the BSs in the $\mathcal{K}_o'$ set by replacing $\mathcal{K}_o$ with $\mathcal{K}_o'$ in $\text{P3}$, and solving $\text{P3}$ using off-the-shelf linear programming solver.

% % \State \textbf{Output:} Optimal transmit power of the BSs, $\{P_k^*\}$.

% % \end{algorithmic}
% % \end{algorithm}











% \begin{thebibliography}{8}
% \bibitem{12GHz_WCL}
% T. R. Niloy \textit{et al.}, ``Interference analysis of coexisting 5G networks and NGSO FSS receivers in the 12 GHz band,'' \textit{IEEE Wireless Commun. Lett.} (early access)

%  \bibitem{12GHz_ComMag}
% Z. Hassan \textit{et al.}, ``Spectrum sharing of the 12 GHz band with two-way terrestrial 5G mobile services: Motivations, challenges, and research road map,'' \textit{IEEE Commun. Mag.} (early access).

% \bibitem{OpenCellId}
% https://www.openstreetmap.org/\#map=4/38.01/-95.84.

% \bibitem{SpaceXanalysis}
% SpaceX, ``Spacex analysis of the effect of terrestrial mobile deployment
% on NGSO FSS downlink operations, ''  Tech. Rep., June. 2022.

% \bibitem{RKFreport}
% RKF Eng. Solutions, ``Assessment of feasibility of coexistence between NGSO FSS earth stations and 5G operations in the 12.2–12.7 GHz band,'' Tech. Rep., May 2021.

% \bibitem{pathloss}
% ETSI, ``5G; Study on channel model for frequencies from 0.5 to 100 GHz,'' 3GPP TR 38.901 version 14.0.0 Release 14.

% \bibitem{Hattab2018InterferenceAO}
% G. Hattab \textit{et al.}, ``Interference analysis of the coexistence of 5G cellular networks with satellite earth stations in 3.7-4.2 GHz,'' \textit{IEEE International
% Conference on Communications Workshops}, 2018 pp. 1–6.

% \bibitem{Balanis}
% Balanis, C.A. (2016) Antenna theory: Analysis and design. Hoboken, NJ: Wiley. 

% \bibitem{PL_Rain}
% Singh, H., Kumar, V., Saxena, K. et al. Proposed Model for Radio Wave Attenuation due to Rain (RWAR). Wireless Pers Commun 115, 791–807 (2020). https://doi.org/10.1007/s11277-020-07598-3


% \bibitem{popuden}
% United States Census Bureau, [Online]. Available: https://www.census.gov/quickfacts/fact/table/blacksburgtownvirginia.

  
% \end{thebibliography}





% \end{document}
